FLTracer: Accurate Poisoning Attack Provenance in Federated Learning

Federated Learning (FL) is a promising distributed learning approach that enables multiple clients to collaboratively train a shared global model. However, recent studies show that FL is vulnerable to various poisoning attacks, which can degrade the performance of global models or introduce backdoors into them. In this paper, we first conduct a comprehensive study on prior FL attacks and detection methods. The results show that all existing detection methods are only effective against limited and specific attacks. Most detection methods suffer from high false positives, which lead to significant performance degradation, especially in not independent and identically distributed (non-IID) settings. To address these issues, we propose FLTracer, the first FL attack provenance framework to accurately detect various attacks and trace the attack time, objective, type, and poisoned location of updates. Different from existing methodologies that rely solely on cross-client anomaly detection, we propose a Kalman filter-based cross-round detection to identify adversaries by seeking the behavior changes before and after the attack. Thus, this makes it resilient to data heterogeneity and is effective even in non-IID settings. To further improve the accuracy of our detection method, we employ four novel features and capture their anomalies with the joint decisions. Extensive evaluations show that FLTracer achieves an average true positive rate of over $96.88\%$ at an average false positive rate of less than $2.67\%$, significantly outperforming SOTA detection methods. \footnote{Code is available at \url{https://github.com/Eyr3/FLTracer}.}

==> 4feasibility.tex <==

\section{Feasibility Study and New Evasion Attacks} 
\label{sec:attackfeasibility}

In this section, we study the feasibility of existing attacks. We first introduce the experimental setup, including the datasets, model structures, and parameters. Then we introduce nine attack performance metrics employed in our evaluation. Specifically, we aim to answer the following research questions: \\
% $\bullet$
$\blacksquare$  \textit{RQ1:} How effective, efficient, and robust are the existing untargeted and targeted attacks under FL?  \\
% How do different factors affect the attacks in federated learning?  
% \item \textit{RQ2:} How do different attack strategies affect attack performance?
$\blacksquare$  \textit{RQ2:} How effective are the existing detection and defense methods against poisoning attacks? \\
$\blacksquare$  \textit{RQ3:} Are there other evasion attacks that can circumvent existing detection methods?
%$\blacksquare$ 
% \vspace{-4mm}
% \begin{itemize}
% \setlength{\itemsep}{0pt}
% \setlength{\parsep}{0pt}
% \setlength{\parskip}{0pt}
%     \item \textit{RQ1:} How effective, efficient, and robust are the existing untargeted and targeted attacks under FL?  
%     % \vspace{-2mm}
%     % How do different factors affect the attacks in federated learning?  
%     % \item \textit{RQ2:} How do different attack strategies affect attack performance?
%     \item \textit{RQ2:} How effective are the existing detection and defense methods against poisoning attacks? 
%     % \vspace{-2mm}
%     \item \textit{RQ3:} Are there other evasion attacks that can circumvent existing detection methods?
%     % \vspace{-2mm}
% \end{itemize}



\subsection{Experimental Setup}
\label{sec:setup}
% 

% However, as a SOTA defense against targeted poisoning attacks under FL, DnC~\cite{shejwalkar2021manipulating} utilizes SVD to effectively detect and remove malicious clients despite high false positives. 


% We evaluate 13 types of attacks in untargeted setting and 8 types of attacks in targeted setting. Untargeted attacks are evaluated on MNIST~\cite{lecun1998gradient}, EMNIST~\cite{cohen2017emnist} and CIFAR10~\cite{krizhevsky2009learning}. Targeted attacks are evaluated on CIFAR10 and GTSRB~\cite{Houben-IJCNN-2013} with more complex models. The datasets and model architectures are enumerated in Table~\ref{tab:dataset1}. For dataset MNIST, EMNIST and CIFAR10 and GTSRB, we set the total number of participating clients to 100, 100, 100 and 50. For the integrity of experiments, we measure the performance of attacks both in IID and non-IID setting respectively. In non-IID setting, we use the Dirichlet distribution~\cite{minka2000estimating} with hyperparameter $d=0.5$ to generate data distributions for different clients.


\begin{table}[]
\footnotesize
\setlength\tabcolsep{3pt}
\caption{Datasets, model structures, and parameters}
\vspace{-3mm}
\resizebox{\linewidth}{!}{
\begin{threeparttable}
% \begin{tabular}{@{}c|ccccccc||ccccc@{}}
% \toprule
% \begin{tabular}[c]{@{}c@{}}Attack \\ Type\end{tabular} &
%   Dataset &
%   \begin{tabular}[c]{@{}c@{}}Train\\ inputs\end{tabular} &
%   Class &
%   \begin{tabular}[c]{@{}c@{}}Input \\ size\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}Model \\ structure\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}Data \\ distribution\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}$N$:Total \\ clients\end{tabular} &
% %   \begin{tabular}[c]{@{}c@{}}Attack \\ Round\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}$n$:Clients \\ per round \end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}$m$:Percent of\\ malicious\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}Benign \\ $lr$/epochs\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}Malicious \\ $lr$/epochs\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}Percent of \\ poisoned data\end{tabular} \\ \midrule
% \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}} Un- \\ targeted \end{tabular}} &
%   MNIST &
%   60000 &
%   10 & $28\times28$ &
%   SimpleNet &
%   IID &
%   100 &
%   \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}} 10 \\ MTB:20\\ Fang:20\end{tabular}} &
%   20\% &
%   0.01/2 &
%   0.01/2 &
%   \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}} 0\% \\ DLA:5\%\end{tabular}} \\
% \multicolumn{1}{c|}{} &
%   EMNIST &
%   73168 &
%   47 & $28\times28$ &
%   SimpleNet &
%   non-IID &
%   100 &
%   &
%   20\% &
%   0.01/2 &
%   0.01/2 &
%   \\
% \multicolumn{1}{c|}{} &
%   \multirow{2}{*}{CIFAR10} &
%   \multirow{2}{*}{50000} &
%   \multirow{2}{*}{10} & \multirow{2}{*}{$32\times32$} &
%   AlexNet &
%   IID\&non-IID &
%   100 &
%   &
%   20\% &
%   0.1/2 &
%   0.1/2 &
%   \\
% \multicolumn{1}{c|}{} &
%   &
%   &
%   &
%   &
%   ResNet18 &
%   IID\&non-IID &
%   100 &
%   &
%   20\% &
%   0.1/2 &
%   0.1/2 &
%   \\ \midrule
%   \multirow{4}{*}{Targeted^{*}} &
%   HAR & 
%   7353 & 
%   6 & $1\times 561$ &
%   DNN &
%   non-IID &
%   30 &
%   10 &
%   20\% &
%   0.01/2 &
%   0.005/4 &
%   3\% \\
%   \multicolumn{1}{c|}{} &
% % \multicolumn{1}{c|}{\multirow{3}{*}{Targeted}} &
%   \multirow{2}{*}{CIFAR10} &
%   \multirow{2}{*}{50000} &
%   \multirow{2}{*}{10} & \multirow{2}{*}{$32\times32$} &
%   ResNet18 &
%   IID\&non-IID &
%   100 &
%   10 &
%   \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}10\% \\ DBA:20\%\end{tabular}} &
%   0.01/2 &
%   0.005/6 &
%   3\%\\
% \multicolumn{1}{c|}{} &
%   &
%   &
%   &
%   &
%   VGG16 &
%   IID\&non-IID &
%   100 &
%   10 &
%   &
%   0.01/2 &
%   0.005/6 &
%   3\% \\
% \multicolumn{1}{c|}{} &
%   GTSRB & 
%   39209 & 
%   43 & $32\times32$ &
%   ResNet34 &
%   IID\&non-IID &
%   50 &
%   10 &
%   &
%   0.01/2 &
%   0.005/4 &
%   3\% \\ \bottomrule
% \end{tabular}
\begin{tabular}{@{}c|ccccccc@{}}
\toprule
\begin{tabular}[c]{@{}c@{}} \end{tabular} &
  Dataset &
%   \begin{tabular}[c]{@{}c@{}}Train\\ inputs\end{tabular} &
%   Class &
%   \begin{tabular}[c]{@{}c@{}}Input \\ size\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Model \\ structure\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Data \\ distribution\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}$N$\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}Attack \\ Round\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}$n$\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}$P_m$\end{tabular} & %Percent of\\ malicious
%   \begin{tabular}[c]{@{}c@{}}Benign \\ $lr$/epochs\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}Malicious \\ $lr$/epochs\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}$P_p$\end{tabular} \\ \midrule %Percent of \\ poisoned data
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}} Un- \\ targeted \end{tabular}} &
  MNIST &
%   60000 &
%   10 & $28\times28$ &
  SimpleNet &
  IID &
  100 &
  \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}} 10 \\ MTB:20\\ Fang:20\end{tabular}} &
  20\% &
%   0.01/2 &
%   0.01/2 &
  \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}} 0\% \\ DLA:5\%\end{tabular}} \\
\multicolumn{1}{c|}{} &
  EMNIST &
%   73168 &
%   47 & $28\times28$ &
  SimpleNet &
  non-IID &
  100 &
  &
  20\% &
%   0.01/2 &
%   0.01/2 &
  \\
\multicolumn{1}{c|}{} &
  \multirow{2}{*}{CIFAR10} &
%   \multirow{2}{*}{50000} &
%   \multirow{2}{*}{10} & \multirow{2}{*}{$32\times32$} &
  AlexNet &
  IID\&non-IID &
  100 &
  &
  20\% &
%   0.1/2 &
%   0.1/2 &
  \\
\multicolumn{1}{c|}{} &
  &
%   &
%   &
%   &
  ResNet18 &
  IID\&non-IID &
  100 &
  &
  20\% &
%   0.1/2 &
%   0.1/2 &
  \\ \midrule
  \multirow{4}{*}{Targeted} &
  HAR & 
%   7353 & 
%   6 & $1\times 561$ &
  DNN &
  non-IID &
  21 &
  10 &
  20\% &
%   0.01/2 &
%   0.005/4 &
  10\% \\
  \multicolumn{1}{c|}{} &
% \multicolumn{1}{c|}{\multirow{3}{*}{Targeted}} &
  \multirow{2}{*}{CIFAR10} &
%   \multirow{2}{*}{50000} &
%   \multirow{2}{*}{10} & \multirow{2}{*}{$32\times32$} &
  ResNet18 &
  IID\&non-IID &
  100 &
  10 &
  \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}10\% \\ DBA:20\%\end{tabular}} &
%   0.01/2 &
%   0.005/6 &
  3\%\\
\multicolumn{1}{c|}{} &
  &
%   &
%   &
%   &
  VGG16 &
  IID\&non-IID &
  100 &
  10 &
  &
%   0.01/2 &
%   0.005/6 &
  3\% \\
\multicolumn{1}{c|}{} &
  GTSRB & 
%   39209 & 
%   43 & $32\times32$ &
  ResNet34 &
  IID\&non-IID &
  50 &
  10 &
  &
%   0.01/2 &
%   0.005/4 &
  3\% \\ \bottomrule
\end{tabular}
\begin{tablenotes}
%     %\item [1] Attack rounds of targeted attacks in GTSRB in IID and non-IID setting is 101-200 and 201-300, respectively.
\item{We refer the readers to Table~\ref{tab:dataset1} for the complete parameter settings. ($N$: Total clients; $n$: Clients per round; $P_m$: Percent of malicious clients; $P_p$: Percent of poisoned data)}
% \item{$^*$The parameters of the targeted attack apply to both A-M and A-BM attacks. In the A-S attack, the adversary attacks for one round and scales the updates by 10$\times$.} %performs in the first round of attack, with one malicious client.
\end{tablenotes}
\end{threeparttable}
}
\vspace{-4mm}
\label{tab:dataset}
\end{table}



\textbf{Datasets and model structures:} We use five datasets (including four image classification datasets and a human activity recognition dataset) and six model structures.
Datasets include MNIST~\cite{lecun1998gradient}, EMNIST~\cite{cohen2017emnist}, Human activity recognition (HAR)~\cite{anguita2013public}, CIFAR10~\cite{krizhevsky2009learning}, and GTSRB~\cite{Houben-IJCNN-2013}. Model structures contain DNN (2 fully connected layers (FC)), SimpleNet (2 convolutional layers and 2 FC), AlexNet~\cite{krizhevsky2012imagenet}, ResNet18~\cite{he2016deep}, VGG16~\cite{simonyan2014very}, and ResNet34~\cite{he2016deep}. We summarize the datasets, number of training inputs, number of classes, input size, and model structures in Table~\ref{tab:dataset1} (columns 2-6). 

We generate the data distribution of $N$ clients in IID and non-IID settings for all datasets. %, as summarized in columns 7-8. 
Following the setup in~\cite{shejwalkar2021back, bagdasaryan2020backdoor, xie2019dba}, we use a Dirichlet distribution~\cite{minka2000estimating} with $d=0.5$ to simulate the real non-IID settings. We refer to the code in \cite{bagdasaryan2020backdoor, bagdasaryan2020blind} to split the labels and the data of the dataset, as shown in Fig.~\ref{fig:data_distribution}. For HAR collected from the smartphone sensors of 30 real-world users, we consider each user to be a client.
% Following the setup in~\cite{shejwalkar2021back, bagdasaryan2020backdoor, xie2019dba}, we use a Dirichlet distribution~\cite{minka2000estimating} with $d=0.5$ to simulate the data distribution in non-IID settings, as shown in Fig.~\ref{fig:data_distribution}. 

\noindent \textbf{Learning parameters:} 
We set up the standard training process using an SGD optimizer for local training, and the global learning rate is $\eta=1/n$.
Table~\ref{tab:dataset1} (columns 9-13) shows the number of selected clients each round, percentage of malicious clients, benign $lr$/epochs, malicious $lr$/epochs, and percentage of poisoned data. 
% Here malicious $lr$/Epochs is different from benign $lr$/epochs because malicious clients can modify hyperparameters to attack more effectively. 
% Malicious $lr$/Epochs can be modified to attack more effectively.
We launch untargeted attacks at the beginning of training and targeted attacks in the 200th round of training, since targeted attacks are more effective after the model convergences~\cite{bagdasaryan2020backdoor}. 
More details are summarized in $\S$~\ref{sec:expsetup}.

% \textbf{Attacks:}
% For untargeted attacks, we evaluate six types of classical attacks (i.e., an add noise attack, a sign-flipping attack, and three dirty label attacks) and eight types of evasion attacks (i.e., six MTB attacks~\cite{shejwalkar2021manipulating} and two Fang attacks~\cite{2019Local}), as summarized in Table~\ref{tbl:attacks} (rows 2-3). 
% For targeted attacks, we evaluate eight types of attacks, including three types of backdoor triggers (i.e., $3\times3$ grid trigger in BadNets~\cite{gu2017badnets} (BN), random noise trigger in Blend~\cite{chen2017targeted} (BL), and $1\times6$ distributed trigger in DBA~\cite{xie2019dba} (DB)) and three types of injection strategies (i.e., single-attack (A-S), multiple-attack (A-M), and blind multiple-attack (A-BM)), as summarized in Table~\ref{tbl:attacks} (rows 4-5). 

\noindent \textbf{Attacks and detection methods:}
As summarized in Table~\ref{tab:attacktax1} (column 3), we evaluate 14 types of untargeted attacks and 16 types of targeted attacks. We detect untargeted and targeted attacks by three different detection and defense methods: DnC~\cite{shejwalkar2021manipulating}, Median~\cite{yin2018byzantine}, and Fine-pruning~\cite{liu2018fine}, which represent gradient anomaly detection method, Byzantine-robust aggregation, and model sanitization method, respectively. 
We use three levels (i.e., high, medium, and low) to measure the effectiveness of the detection methods. \textit{High} indicates that the method is effective in detection, i.e., it achieves a high TPR at a low FPR. \textit{Low} indicates that the method performs poorly in detection, i.e., it achieves high FPR when TPR is high. The \textit{Medium} detection effectiveness is between \textit{high} and \textit{low}.


% \begin{table}[]
% % \footnotesize
% \centering
% \caption{Summary of attacks}
% \vspace{-2mm}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{ll}
% \toprule
% \multicolumn{1}{l}{No attack} &
%   B: Baseline \\ \midrule
%   \begin{tabular}[c]{@{}l@{}}Untargeted\\ classical\end{tabular} &
%   \begin{tabular}[c]{@{}l@{}}C-A: Add Noise; C-B: Sign-flipping;  C-C: (DLA)FIX-FIX; \\ C-D: (DLA)FIX-RNG; C-E: (DLA)RNG-FIX; C-F: (DLA)RNG-RNG.\end{tabular} \\ %\cmidrule(l){2-2}
% \midrule
%   \begin{tabular}[c]{@{}l@{}}Untargeted\\ evasion\end{tabular} &
%   \begin{tabular}[c]{@{}l@{}}E-A: MTB\_Mkrum; E-B: MTB\_Bulyan; E-C: MTB\_Median; \\ E-D: MTB\_Trmean; E-E: MTB\_Min-Max; E-F: MTB\_Min-Sum;\\ E-G: Fang\_Mkrum; E-H: Fang\_Trmean.\end{tabular} \\ %\cmidrule(l){2-2} 
% \midrule
%   \begin{tabular}[c]{@{}l@{}}Targeted\\ classical\end{tabular} &
%   Trigger: BN, BL, BD; Inject: A-S, A-M, A-BM. \\ %\cmidrule(l){2-2} 
% \midrule
%   \begin{tabular}[c]{@{}l@{}}Targeted\\ evasion\end{tabular} &
%   \begin{tabular}[c]{@{}l@{}}Trigger: BN, BL, BD; Inject: A-S, A-M, A-BM.\\ Combine with convolution replacement strategy.\end{tabular} \\ \bottomrule
% \end{tabular}
% }
% \label{tbl:attacks}
% \vspace{-5mm}
% \end{table}


\subsection{Evaluation Metrics} 
\label{sec:metrics}
Table~\ref{tab:performance_metrics} shows nine metrics to evaluate the performance of the normal task and backdoor task under the attack from three aspects, including effectiveness, stability, and robustness. For the normal task, we use accuracy ($ACC$) and model stability ($MS$) to measure the effectiveness and stability of the global model as a whole.  The clean accuracy drop ($CAD$) is introduced to measure the effectiveness of the attack. Particularly, we introduce a group of category metrics to further evaluate the effectiveness and stability of untargeted attacks, including category accuracy ($CA$), worst category accuracy ($WCA$), best category accuracy ($BCA$), and category accuracy stability ($CAS$). 
Lower $ACC$, $BCA$, and $WCA$ indicate stronger attacks, and higher $CAD$, $MS$, and $CAS$ indicate stronger attacks.
For the backdoor task, we utilize the attack success rate ($ASR$) to evaluate the effectiveness of targeted attacks. To further evaluate the robustness of the backdoor injection, we incorporate backdoor injection rounds ($BIR$) and backdoor removal rounds ($BRR$) to measure the speed of backdoor injection and disappearance. Higher $ACC$, $ASR$, and $BRR$ indicate stronger attacks, and lower $BIR$ and $MS$ imply stronger attacks.

% We employ nine metrics (as shown in Table~\ref{tab:performance_metrics}) to evaluate the effectiveness and robustness of attacks. We use accuracy ($ACC$) and model stability ($MS$) to measure the impact of each attack on the global model.
% For untargeted attacks, clean accuracy drop ($CAD$) and Category accuracy ($CA$) measure the effectiveness of the attack, i.e., the impact on the global model accuracy. 
% We incorporate three category metrics: worst category accuracy ($WCA$), best category accuracy ($BCA$), and category accuracy stability ($CAS$). Lower $ACC$, $BCA$, and $WCA$ indicate stronger attacks, while higher $CAD$, $MS$, and $CAS$ indicate stronger attacks. 
% For targeted attacks, we use the attack success rate ($ASR$) to evaluate the effectiveness of the backdoor injection. In addition, we observe that the speed of backdoor injection and the speed of backdoor disappearance after the attack vary significantly across attacks. We incorporate backdoor injection rounds ($BIR$) and backdoor removal rounds ($BRR$) to measure the robustness of the backdoor attacks. Higher $ACC$, $ASR$, and $BRR$ indicate stronger attacks, while lower $BIR$ and $MS$ imply stronger attacks.
%  and to evaluate the velocity of backdoor implantation and the natural disappearance speed of backdoors during normal training with terminating attacks. 

\begin{table}[]
\setlength\tabcolsep{3pt}
\centering
% \small
\caption{Evaluation metrics}
\vspace{-3mm}
\resizebox{\linewidth}{!}{
\begin{threeparttable}  
\begin{tabular}{@{}ll@{}}
\toprule
Metrics      & Definition               \\ % & Demand
% \hline
% \hline
\midrule
(E) \textit{ACC} & \begin{tabular}[c]{@{}c@{}}\#correct\ predictions / \#total\ predictions \end{tabular}                \\ %& High
(S)  \textit{MS} &
  \begin{tabular}[c]{@{}c@{}} Standard deviation of $ACC$ \end{tabular} \\ %, \\ Accuracy stability &Low  for the last ten rounds \(\sqrt{\frac{1}{10}\sum_{r\in[\rho]}(ACC^r-\overline{ACC})^2}\)
% \hline 
% \midrule
(E) \textit{CAD} & Drop in $ACC$ of clean inputs after the attack \\
(E)  $CA_c$ &
  \begin{tabular}[c]{@{}c@{}} \#correct\ predictions\ of\ class\ $c$ / \#total\ predictions\ of\ class\ $c$ \end{tabular}  \\ %,\\ Accuracy on category & High
(E) \textit{WCA} & Minimum $CA_c$ in all categories  \\ %, \\ Worst category accuracy  &  High \(\min\limits_{c\in[m]}CA_c\), where $m$ is the total number of categories
(E) \textit{BCA} & Maximum $CA_c$ in all categories \\
  %\begin{tabular}[c]{@{}c@{}}\(\max\limits_{c\in[m]}CA_c\)\end{tabular}, where $m$ is the total number of categories  \\ %, \\ Best category accuracy & High
(S) \textit{CAS} &
  \begin{tabular}[c]{@{}c@{}} Standard deviation of $CA$ of all categories \end{tabular} \\  %, \\ Category accuracy stability & Low    \(\sqrt{\frac{1}{10}\sum_{r\in[\rho],c\in[m]}(CA_c^r-\overline{CA})^2}\) for the last ten rounds
% \hline 
% \midrule
(E) \textit{ASR} &  \#correct \ poisoned \ predictions / \#total\ poisoned \ predictions  \\ % & High
(R) \textit{BIR} & Number of rounds to reach 90\% \textit{ASR} \\ % & 
(R) \textit{BRR} & Number of rounds to remove backdoors when training with clean data \\%& High   \multirow{1}{*}{\begin{tabular}[c]{@{}l@{}}\\ (reach the benchmark $ASR$) \\ \end{tabular}} 
\bottomrule
\end{tabular}
\begin{tablenotes}
    \item{(E)-Effectiveness; (S)-Stability; (R)-Robustness}
\end{tablenotes}
\end{threeparttable}
}
\vspace{-5mm}
\label{tab:performance_metrics}
\end{table}


% !!!!!!!!!!!! The following are the evaluation criteria. For untargeted attacks, in terms of global models performance, an excellent attack requires a significant drop in $ACC$ and an increase in $MS$, or worse $BCA/WCA$ and $CAS$ to widen the performance gap among categories as much as possible. For targeted attacks, adversaries expect that $ASR$ will be as high as possible, backdoors are implanted fast, last for a longer time, and are hard to eliminate, which is manifested in smaller $BIR$ and larger $BRR$. At the same time, adversaries expect the performance of main tasks in global models to be unaffected, which is consistent with the requirements of benign clients. Therefore, it is necessary to keep high $ACC$ and low $MS$.


% Note that, we report mainly results on CIFAR10 (ResNet18) in non-IID settings due to space constraints, and we postpone other results to Appendix~\ref{sec:appendix_evaluation}. 


\subsection{\textit{RQ1:} Performance of Poisoning Attacks} 
\label{sec:performance_attack}
% add noise attack (C-A), sigh-flipping attack (C-B), FIX-FIX dirty label attack (C-C), MTB attack (E-A to E-F), Fang attack (E-G to E-H)
\textbf{Untargeted attacks:} Fig.~\ref{fig:CAD_un} and Fig.~\ref{fig:CAD_un_1} show the $CAD$ of untargeted evasion and classical attacks on different settings. In non-IID settings, we observe that most untargeted attacks achieve a high $CAD$, except for three dirty label attacks (C-D to C-F). Specifically, the $CAD$ of E-A and C-D on CIFAR10 (AlexNet) are 39.29\% and 0.85\%. 
% On the other hand, most untargeted evasion attacks on MNIST in IID settings can only slow down the training process but not reduce the final model accuracy. 
On the other hand, the performance of untargeted evasion attacks is generally stronger than untargeted classical attacks due to the ability of evasion attacks to generate optimized perturbations. The average $CAD$ for evasion and classical attacks is 25.8\% and 3.77\%.

Next, we report $ACC$, $MS$, $WCA$, $BCA$, and $CAS$ of untargeted evasion and classical attacks, as shown in Fig.~\ref{fig:robustness_un} and Fig.~\ref{fig:robustness_un_1}. We observe that untargeted classical attacks mainly affect the stability of the model. Specifically, the $MS$ for C-C attack is 4.15, much higher than the baseline (0.7). Moreover, untargeted evasion attacks significantly affect the $ACC$ and $CA$. The $ACC$ and $CA$ of E-A to E-G are smaller than the baseline by 41.82\% and 41.15\%, respectively. We also report the results of other datasets in Fig.~\ref{fig:robustness_un_iid} and Fig.~\ref{fig:robustness_un_noniid}.
% the results on ResNet18 trained on CIFAR10 in non-IID settings


% \begin{figure}[]
%   \centering
% %   \vspace{-3mm}
%   \subfigure[Untargeted classical attacks]{
%   \includegraphics[width=0.86\linewidth]{./figures/untarget_cl_feasi_CAD}
%   }\vspace{-1mm}
%   \subfigure[Untargeted evasion attacks]{
%   \includegraphics[width=0.86\linewidth]{./figures/untarget_ea_feasi_CAD}
%   }
%   \vspace{-2mm}
%   \caption{The clean accuracy drop of untargeted attacks under different datasets, model architectures, and data distribution. In (a), the clean accuracy drop of sign-flipping attacks on EMNIST in non-IID settings is 81.28\% (over 20\%).
%   In (b), the clean accuracy drop for all attacks on MNIST in IID settings is less than 0.2\%.} %. The left part is the IID and the right part is the non-IID
%   \label{fig:CAD_un}
%   \vspace{-5mm}
% \end{figure}
\begin{figure}[]
  \centering
%   \vspace{-3mm}
  \includegraphics[width=0.87\linewidth]{./figures/untarget_ea_feasi_CAD}
  \vspace{-3mm}
  \caption{The $CAD$ of untargeted evasion attacks. $CAD$ for all attacks on MNIST in IID settings is less than 0.2\%.}
  \label{fig:CAD_un}
  \vspace{-5mm}
\end{figure}


% \begin{figure}[]
%   \centering
% %   \vspace{-2mm}
%   \subfigure[Untargeted classical attacks compared with baseline (B)]{
% %   \vspace{-2mm}
%   \includegraphics[width=0.8\linewidth]{./figures/untarget_cl_feasi_noniid_robust}
%   }\vspace{-1mm}
%   \subfigure[Untargeted evasion attacks compared with baseline (B)]{
%   \includegraphics[width=0.8\linewidth]{./figures/untarget_ea_feasi_noniid_robust}
%   }
%   \vspace{-2mm}
%   \caption{The accuracy and category accuracy of untargeted attacks and on CIFAR10 (ResNet18) in non-IID settings. Untargeted classical and evasion attacks mainly affect the stability and accuracy of the model, respectively.}
%   \label{fig:robustness_un}
%   \vspace{-5mm}
% \end{figure}
\begin{figure}[]
    % \vspace{-3mm}
  \centering
  \includegraphics[width=0.8\linewidth]{./figures/untarget_ea_feasi_noniid_robust}
  \vspace{-3mm}
  \caption{$ACC$ and $CA$ for untargeted evasion attacks on CIFAR10 (ResNet18) compared to baseline (B) (non-IID).}
  \label{fig:robustness_un}
  \vspace{-6mm}
\end{figure}

\vspace{-2mm}
\begin{center}
\fcolorbox{darkblue}{gray!10}{\parbox{.96\linewidth}{\textbf{\textcolor{darkblue}{Remark 1}}. The 14 untargeted attacks (except for C-D to C-F) pose a variety of substantial threats to FL.}}
\end{center}
\vspace{-2mm}

\textbf{Targeted attacks:} 
Fig.~\ref{fig:ASR_tar_1} shows $ASR$ of eight targeted attacks on different settings. We observe that most attacks can inject backdoors with a nearly 100\% $ASR$, except for BN(A-S) and BL(A-S) attacks on GTSRB in non-IID settings. For different attack strategies, A-S is more difficult to inject backdoors compared to A-M and A-BM because A-S only injects a single round. For different datasets, a dataset with fewer categories and more data inputs is easier to inject backdoors. Specifically, the average $ASR$ on CIFAR10 is 96.21\%, which is higher than 76.11\% for GTSRB. We also observe that the backdoor injection is unstable and slow at the beginning of the training, as shown in Fig.~\ref{fig:asr_0_200}. Due to the low accuracy of the global model, it is difficult to converge the global model and inject backdoors into it simultaneously. %, backdoors can be injected more quickly and successfully when the model is converged. 
% A general strategy for backdoor attacks is to train as a benign client at the beginning of the training and launch the attack after model convergence.


% \textbf{Efficiency and robustness of targeted attacks:}
Fig.~\ref{fig:Robustness_tar}(a) shows the $BIR$ and $BRR$ of eight targeted attacks. We observe that most attacks can inject backdoors with an $ASR$ of over 90\% in less than 100 rounds, e.g., only 14 rounds in BN(A-M). Moreover, the $BRR$ usually exceeds 200 rounds, except for A-S attacks. In an A-S attack, the adversary injects a backdoor for one round, and the global model takes more than 57 rounds to remove the backdoor. 
%The low number of backdoor injection rounds and the high number of $BRR$ imply that backdoor attacks are robust under FL, posing a significant security risk to FL. We also report the results for other datasets.
The small $BIR$ and the large $BRR$ imply that these attacks are robust, posing a significant security risk to FL. We also report the results for other datasets (see Fig.~\ref{fig:Robustness_tar_iid} (IID) and Fig.~\ref{fig:Robustness_tar_noniid} (non-IID)).

\vspace{-2mm}
\begin{center}
\fcolorbox{darkblue}{gray!10}{\parbox{.96\linewidth}{\textbf{\textcolor{darkblue}{Remark 2}}. The 8 classical targeted attacks can successfully inject backdoors. When the global model converges, backdoors can be injected more quickly and successfully, similar to the conclusion in \cite{bagdasaryan2020backdoor}.}} %, and the backdoor injection rounds are proportional to the backdoor removal rounds.
\end{center}
\vspace{-2mm}
% \textbf{Takeaway 1.} 
% All attacks considered (14 untargeted attacks and 8 classical targeted attacks, except for C-D to C-F) pose a substantial threat to FL. 


% \begin{figure}[]
%   \centering
% %   \vspace{-3mm}
%   \subfigure[Targeted classical attacks]{
%   \includegraphics[width=0.9\linewidth]{./figures/target_cl_feasi_ASR}
  
%   }\vspace{-1mm}
%   \subfigure[Targeted evasion attacks]{
%   \includegraphics[width=0.9\linewidth]{./figures/target_ea_feasi_ASR}
%   }
%   \vspace{-2mm}
%   \caption{Attack success rate of targeted attacks under different datasets, model structures, and data distribution. }
%   \label{fig:ASR_tar}
%   \vspace{-5mm}
% \end{figure}



\begin{figure}[]
  \centering
%   \vspace{-3mm}
  \includegraphics[width=\linewidth]{./figures/target_feasi_robust}
  \caption{$BIR$ and $BRR$ for targeted attacks in non-IID settings. A $BIR$ of 200 indicates that more than 200 rounds are required to remove the backdoor. The $BIR$ and $BDR$ assess the efficiency and robustness of targeted attacks, respectively.}
  \label{fig:Robustness_tar}
  \vspace{-4mm}
\end{figure}



\subsection{\textit{RQ2:} Effectiveness of Existing Detection} 
\label{sec:defense_eff}

\textbf{Untargeted attacks:} We find that existing methods can effectively detect untargeted attacks in IID settings, as shown in Fig.~\ref{fig:resist_iid}. However, the detection effectiveness in non-IID settings is unstable, as shown in Fig.~\ref{fig:resist}(a) and (b). DnC is effective for only several specific attacks, such as C-A, E-C, and E-D, but has low effectiveness for other attacks. The effectiveness of Median is generally low in non-IID settings because Median can only guarantee convergence of FL, but this is insufficient to detect malicious clients.

\textbf{Targeted attacks:} We find that the effectiveness of DnC is generally high in IID settings, as shown in Fig.~\ref{fig:resist_iid}. However, the effectiveness of DnC and Fine-pruning is generally low in non-IID settings, as shown in Fig.~\ref{fig:resist}(c). The low performance of Fine-pruning is because the server under FL does not have a large dataset to fine-tune the model, resulting in a significant decrease in the classification accuracy of the global model. 
DnC has high effectiveness only in A-S and BN(A-M) attacks but has low effectiveness in A-BM attacks due to the stealthiness of blind backdoor attacks. 

\begin{figure}[]
  \centering
  % \vspace{-7mm}
  \includegraphics[width=0.96\linewidth]{./figures/feasibility_defense_effect}
  \vspace{-3mm}
  \caption{Effectiveness of existing detection methods against attacks in non-IID settings (H:high; M:medium; L:low).}
  %We apply DnC and Median against untargeted attacks. We apply DnC and Fine-pruning against targeted attacks.} %CIFAR10, ResNet18
  \vspace{-6mm}
  \label{fig:resist}
\end{figure}


%We apply DnC and Fine-pruning to evaluate the effectiveness of existing methods. 
%We apply Median and DnC to evaluate the effectiveness of existing detection methods.
% Median prevents a global model from collapsing due to sign-flipping attacks on EMNIST. But for CIFAR10 (ResNet18), untargeted classical attacks that have a slightly negative impact on global model performance, can easily resist Byzantine-robust aggregations. As evasion attacks against them, MTB and Fang attacks have high resistance. 
% For untargeted classical attacks, sign-flipping and dirty label attacks both have high resistance, but due to the weak attack effect, add noise attack is hard to resistant the detection of DnC. Except for MTB Median and Trmean attacks, evasion attacks are easily resistant to DnC. 


% feasibility of targeted classical attacks. \textbf{For all combinations of trojan triggers and training methods, backdoors can be successfully implanted in FL settings}, where $ASR$s reach nearly 100\%. On the one hand, for different trigger types, the difference of $BIR$ manifests the ranking of trigger implantation difficulty is: BN<BL<DB. In addition, the $BRR$ of BL in A-S is lower than that of BN, implying that the attack robustness of BL is worse than that of BN, and the results of A-M shown in Fig.~\ref{fig:acc_backdoor_cifar} of Appendix~\ref{} also validate this observation. In A-S attack using DB, a backdoor can not be implanted into a global model when the global model learning rate is 0.1. Therefore, we follow the setting in ~\cite{xie2019dba}, where the global model learning rate is 0.01. That implies that the global model learning rate plays a role part in A-S (DB) attacks. Furthermore, despite using BL to initiate backdoor injection at a higher $ASR$, $ASR$ in BN reaches a peak faster than that in BL. When terminating the attack at round 400, $ASR$ drops faster in the global model with BL, implying a lack of robustness and stability. In conclusion, \textbf{random noise triggers (BL) are less effective and stable than other triggers}. On the other hand, comparing different backdoor training methods, we observe that \textit{ACC} in A-BM is higher than \textit{MS} slightly in A-M. Besides, the detection results of targeted poisoning attacks are shown in Sec.~\ref{sec:backdoor_evaulation}, where $TPR$ in A-BM attack is lower than that of A-M attack, indicating that A-BM attack makes the backdoor injection process more stealthy. Therefore, \textbf{using blind multiple-shot attack has better results for backdoor implantation in FL settings}.


% Add noise attack has a limited effect on \textit{ACC} for the global model, which mainly influences \textit{BCA} by nearly 5\% decreased. Sign-flipping attack leads to \textit{ACC} by 7.7\% lower on CIFAR10 (ResNet18). For dirty label attack, strategy has an essential impact on the attack effect. For DLA on CIFAR10, FIX-FIX strategy resulted in a nearly 10\% drop in \textit{ACC} and a 2X increase in \textit{MS} over the baseline, but the other strategies slightly affect the global model. This is because randomness results in the attenuation of the attack effect. Therefore, FIX-RNG (C-D), RNG-FIX~(C-E), and RNG-RNG (C-F) are not included in subsequent detection evaluation. 
% For a simple model structure and dataset, i.e. EMNIST task, Sign-flipping attack has a wider impact on the global model. 

% Table~\ref{tab:fea_evasion_un} shows the feasibility of untargeted evasion attacks. MTB attack is effective against four Byzantine-robust aggregations, with undermining exceeding 40\%, 30\%, and 40\% for $ACC$, $BCA$, and $WCA$, respectively. Specifically, E-A attack has the most severe impact on the stability of the model, whose $MS$ increases 3X. In E-D attack, $ACC$ is the same as random guessing at only 10.33\% and some category accuracy even is 0\%. Furthermore, E-G attack results in a global model collapse with a $ACC$ of only 5.59\%. For E-H attack, the global model drops by 15\% on $ACC$ and increases by 0.6x on $CAS$. 

% Note that, we evaluate the detection against two untargeted evasion attacks in Sec.~\ref{subsec:un_attack_detection}.



% But the detection methods are able only to detect a small proportion of attacks, implying that they can not prevent the backdoor injection, especially for our new evasion attack strategy.

% \vspace{-3mm}
% \begin{center}
% \fcolorbox{darkblue}{gray!10}{\parbox{.96\linewidth}{\textbf{\textcolor{darkblue}{Remark 3}}. Existing detection methods can only ensure high precision in detecting a small fraction of specific attacks and have high false positive rates in non-IID settings.}}
% \end{center}
% \vspace{-2mm}
% \textbf{Takeaway 2.} 
% Existing detection methods can only ensure high precision in detecting a small fraction of attacks and have high false positive rates in non-IID settings. %According to the assessment,


% We evaluate the resistance of targeted attacks against defenses, shown in Table~\ref{tab:resist_tar}. For targeted classical attacks, most attacks have a low resistance to DnC except for A-BM attack. Due to the high stealthy, A-BM attack is hard to detect by DnC. In contrast, Fine-pruning mitigates a backdoor by pruning weights of a poisoned global model, which has a significant negative impact on main tasks. Therefore, considering the performance of main tasks, the resistance to Fine-pruning is commonly higher than to DnC. For our evasion attacks, except for A-S attack, most have excellent resistance to either DnC or Fine-pruning. In A-S attack, the updates of malicious clients are directly amplified with a scale factor, and DnC can easily detect anomalies. Therefore, A-S attack has weak resistance to DnC.

% In Accuracy metrics, \textit{ASR} measures the success of a backdoor attack, \textit{ACC} and \textit{MS} measure the impact of a backdoor attack to the main task. In Attack Robustness metrics, \textit{BIR} and \textit{BRR} measure the quality of a backdoor attack.

\subsection{\textit{RQ3:} A New Targeted Evasion Attack} 
\label{sec:CRBA} 
We discover a new strategy that can combine existing targeted attacks to circumvent gradient anomaly detection. 
We observe that the convolutional layers' weights are more crucial for targeted attacks than other parameters (e.g., the bias and the classifier). Only when the convolutional layers' weights are modified can the backdoor be injected. Thus, we propose a convolution replacement strategy and an existing targeted attack combined with this strategy, called a targeted evasion attack. 
Specifically, the adversary first performs backdoor training and normal training to generate a backdoor model $\theta_B$ and a normal model $\theta_N$, respectively. Then the adversary replaces the convolution weights in $\theta_N$ with those in $\theta_B$ to obtain the new backdoor model $\theta_B^*$. 
\vspace{-2mm}
\begin{center}
\fcolorbox{darkblue}{gray!10}{\parbox{.96\linewidth}{\textbf{\textcolor{darkblue}{Remark 4}}. The critical model updates for targeted attacks are the feature extractor weights, i.e., convolutional layer weights for convolutional neural network (CNN).}}
\end{center}
\vspace{-1mm}

For the effectiveness of this new strategy, we report $ASR$s of eight targeted evasion attacks in Fig.~\ref{fig:ASR_tar}. We find that our new attacks can generally achieve the same effectiveness as the targeted classical attacks. For instance, the average $ASR$ of evasion and classical attacks are 88.3\% and 89.51\% in non-IID settings. For the efficiency and robustness of the new strategy, we report $BIR$ and $BRR$ in Fig.~\ref{fig:Robustness_tar}(b). Our new strategy's average $BIR$ and $BRR$ are close to that of classical attacks ($BIR$: 20.5 vs. 19.4; $BRR$: 158.25 vs. 154.75). 

\begin{figure}[]
  \centering
  \includegraphics[width=0.96\linewidth]{./figures/target_ea_feasi_ASR}
  \vspace{-3mm}
  \caption{The $ASR$ of targeted evasion attacks.}
  \label{fig:ASR_tar}
  \vspace{-6mm}
\end{figure}

% For the effectiveness of existing methods against our new attacks, we report the results in Fig.~\ref{fig:Robustness_tar}(d). We find that our new attacks perform better than classical attacks (c). For instance, in A-M attacks, the effectiveness of DnC is low in our new attacks and is high in classical attacks, indicating that our new attacks are more stealthy. This is because our new attacks modify only the deterministic parameters of updates.

% \vspace{-3mm}
% \begin{center}
% \fcolorbox{darkblue}{gray!10}{\parbox{.96\linewidth}{\textbf{\textcolor{darkblue}{Remark 5}}. Our new evasion strategy is as effective as the classical targeted attack, yet it is stealthier and makes existing detection methods more difficult to detect.}}
% \end{center}
% \vspace{-2mm}
% \textbf{Takeaway 3.}
% The effectiveness of our new attack is similar to that of the classical attack, while our attack is more stealthy and makes existing detection methods more difficult to detect.

% \subsection{Takeaway}\label{sec:attack_takeaway}
% % we summarize some knowledge revealed by our experimental studies, including limitations of existing detection methods for poisoning attacks and 


% From our attack feasibility, for untargeted attacks, a total of 11 attack strategies we evaluated are effective, including add noise (C-A), sign-flipping (C-B), (DLA) FIX-FIX (C-C), MTB (E-A to E-F), and Fang (E-G and E-H) attacks. Most existing detection methods can not effectively detect malicious clients in non-IID settings. For targeted attacks, all 16 evaluated attacks are efficient and robust, including three triggers (BN, BL, DB) and three injection methods (A-S, A-M, A-BM). But the detection methods are able only to detect a small proportion of attacks, implying that they can not prevent the backdoor injection, especially for our new evasion attack strategy.

% 1. Existing untrgeted and targeted attacks are ...
% 2. Existing defense are...

% Next, we display the attack feasibility of CRBA in Table~\ref{tab:fea_evasion_t}. 
%$\theta_B'=\{w_r^*, b_r, w_c, b_c\}$, $=\{w_r^*, b_r^*, w_c^*, b_c^*\}$

% \begin{table}[]
% \footnotesize
% \caption{Attack feasibility of CRBA}
% \vspace{-2mm}
% \begin{tabular}{cl|ccc|cc}
% \toprule
% \multicolumn{2}{c}{Attack Phase}  & \multicolumn{3}{c}{Accuracy} & \multicolumn{2}{c}{Attack robustness} \\
% \cmidrule(lr){1-2} \cmidrule(lr){3-5} \cmidrule(lr){6-7}
% \textbf{Trojan} & \multicolumn{1}{c}{\textbf{Train}} & ACC(\%)  & MS     & \multicolumn{1}{c}{ASR(\%)}  & BIR     & BRR  \\
% \midrule
% \multirow{1}{*}{BN}         & A-S    & 84.29	&0.52	&99.94	&1	&26   \\
% \multirow{1}{*}{BN}         & A-M    & 85.83	&0.84	&100	&31      & 200+ \\
% \multirow{1}{*}{BN}         & A-BM   & 85.46	&1.39	&100	&56      & 200+ \\
% \midrule
% \multirow{1}{*}{BL}         & A-S    & 84.89	&1	&99.99	&1	&40   \\
% \multirow{1}{*}{BL}         & A-M    & 84.81	&0.8	&100	&61 & 200+ \\
% \multirow{1}{*}{BL}         & A-BM   & 85.95	&1.23	&100	&146  & 200+  \\
% \midrule
% \multirow{1}{*}{DB}         & A-S    & 84.35	&0.13	&99.47	&9    & 200+ \\
% \multirow{1}{*}{DB}         & A-M    & 84.92	&1.02	&95.65	&77   & 200+ \\
% \bottomrule
% \end{tabular}
% \label{tab:fea_evasion_t}
% % \vspace{-5mm}
% \end{table}


% \begin{table}[]
% \small
% \caption{Resistance of targeted attacks to existing defenses on non-IID data}
% \begin{tabular}{@{}cccccc@{}}
% \toprule
% \multicolumn{2}{c}{\textbf{Attack Phase}} & \multicolumn{2}{c}{Classical} & \multicolumn{2}{c}{Evasion} \\ \midrule
% \textbf{Trojan} & \textbf{Train}            & DnC  & Fine-pruning                & DnC    & Fine-pruning \\ \midrule
% BN              & \multicolumn{1}{c|}{A-S}  & Low  & \multicolumn{1}{c|}{High}   & Low    & High         \\
% BN              & \multicolumn{1}{c|}{A-M}  & Low  & \multicolumn{1}{c|}{High}   & High   & High         \\
% BN              & \multicolumn{1}{c|}{A-BM} & High & \multicolumn{1}{c|}{High}   & High   & High         \\ \midrule
% BL              & \multicolumn{1}{c|}{A-S}  & Low  & \multicolumn{1}{c|}{Median} & Low    & High         \\
% BL              & \multicolumn{1}{c|}{A-M}  & Low  & \multicolumn{1}{c|}{Median} & High   & High         \\
% BL              & \multicolumn{1}{c|}{A-BM} & High & \multicolumn{1}{c|}{Median} & High   & High         \\ \midrule
% DB              & \multicolumn{1}{c|}{A-S}  & Low  & \multicolumn{1}{c|}{High}   & Low    & High         \\
% DB              & \multicolumn{1}{c|}{A-M}  & Low  & \multicolumn{1}{c|}{Median} & Median & High         \\ \bottomrule
% \end{tabular}
% \end{table}



% \begin{table}[]
% \small
% \vspace{-3mm}
% \caption{Attack Feasibility of Untargeted Classical Attacks}
% \vspace{-4mm}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{cl|ccc|cc}
% % \toprule
%  & \multicolumn{1}{c}{} & \multicolumn{3}{c}{Accuracy} & \multicolumn{2}{c}{Model stability} \\
% \cmidrule(lr){3-5} \cmidrule(lr){6-7}
% No. & \multicolumn{1}{c}{Attack} & ACC(\%)  & BCA(\%) & \multicolumn{1}{c}{WCA(\%)}  & MS & CAS \\
% \midrule
% \multicolumn{1}{l}{}    & \textit{No Attack}    & \textit{73.97}   & \textit{89.00}   & \textit{46.31} & \textit{3.71} & \textit{12.75}  \\
% % \midrule
% C-A             & Add Noise Attack           & 68.41  & \textbf{83.57}   & 48.52  & 3.98 & 11.59  \\
% C-B             & Sign-flipping Attack       & \textbf{66.27}  & 84.38   & 44.32  & 4.00 & 13.28  \\
% % \midrule
% C-C             & (DLA) FIX - FIX            & \textbf{64.33}  & 89.97   & \textbf{39.47}   & \textbf{6.58} & \textbf{16.29} \\
% C-D             & (DLA) FIX - RNG            & 69.43   & 88.38   & \textbf{39.39} & 3.33 & \textbf{15.99}  \\
% C-E             & (DLA) RNG - FIX            & 68.99  & 85.83   & 40.64  & 2.88 & 14.47  \\
% C-F             & (DLA) RNG - RNG            & 69.76   & 87.52   & 48.36  & 4.13& 11.04  \\
% \bottomrule
% \end{tabular}
% }
% \vspace{-3mm}
% \label{tab:fea_cla_un}
% \end{table}



% \begin{figure*}[]
%   \centering
%   \subfigure[Untargeted classical attacks]{
%   \includegraphics[width=0.23\linewidth]{./figures/untarget_cl_feasi_noniid_CAD}
%   }
%   \subfigure[Untargeted evasion attacks]{
%   \includegraphics[width=0.23\linewidth]{./figures/untarget_ea_feasi_noniid_CAD}
%   }
%   \subfigure[Targeted classical attacks]{
%   \includegraphics[width=0.23\linewidth]{./figures/target_cl_feasi_noniid_ASR}
%   }
%   \subfigure[Targeted evasion attacks]{
%   \includegraphics[width=0.23\linewidth]{./figures/target_ea_feasi_noniid_ASR}
%   }
%   \caption{Effectiveness of poisoning attacks}
%   \label{fig:CAD_un}
% \end{figure*}


% \begin{table}[]
% \small

% \caption{Attack Feasibility of Untargeted Evasion Attacks}
% \vspace{-4mm}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{cll|ccc|cc}
% % \toprule
%  & \multicolumn{2}{c}{} & \multicolumn{3}{c}{Accuracy} & \multicolumn{2}{c}{Model stability} \\
% \cmidrule(lr){4-6} \cmidrule(lr){7-8}

% No.         & \multicolumn{1}{c}{Attack}   & \multicolumn{1}{c}{aggregation}    & \multicolumn{1}{c}{ACC(\%)} & BCA(\%) & \multicolumn{1}{c}{WCA(\%)}&  MS    & CAS \\
% \midrule
% \multicolumn{1}{l}{} & \textit{No Attack}            & Mean   & \textit{78.20}   & \textit{93.62}   & \textit{61.59}& \textit{2.08}   & \textit{10.97} \\
% % \midrule
% E-A         & \multirow{1}{*}{MTB\_Mkrum}   & Mkrum  & \textbf{26.91}    & \textbf{57.50}   & \textbf{12.31}& \textbf{6.05}  & 13.32 \\
% E-B         & \multirow{1}{*}{MTB\_Bulyan} & Bulyan & \textbf{19.15}   & \textbf{52.09}   & \textbf{2.65}& 2.82    & 14.33 \\
% E-C         & MTB\_Median            & Median & \textbf{22.49}   & \textbf{47.43}   & \textbf{3.79}& 3.03    & 12.80 \\
% E-D         & MTB\_Trmean            & Trmean & \textbf{10.33}   & \textbf{59.34}   & \textbf{0.00}& 0.38    & \textbf{17.48} \\
% E-E         & MTB\_Min-Max           & Bulyan & \textbf{13.46}   & \textbf{25.32}   & \textbf{0.05} & 3.01   & 8.54 \\
% E-F         & MTB\_Min-Sum           & Mkrum  & \textbf{36.38}   & \textbf{57.48}   & \textbf{20.46}& 2.98   & 11.36 \\
% % \midrule
% E-G         & \multirow{1}{*}{Fang Attack} & Mkrum  & \textbf{5.59}   & \textbf{16.90}   & \textbf{0.01}   & 1.07   & 5.38 \\
% E-H         & \multirow{1}{*}{Fang Attack} & Trmean & \textbf{64.20}   & 85.19   & \textbf{33.89} & 3.06  & \textbf{16.13} \\
% \bottomrule
% \end{tabular}
% }
% \vspace{-4mm}
% \label{tab:fea_evasion_un}
% \end{table}

% \begin{table}[]
% \footnotesize
% \caption{Attack feasibility of targeted classical attacks}
% \vspace{-2mm}
% \begin{tabular}{cl|ccc|cc}
% \toprule
% \multicolumn{2}{c}{Attack Phase}  & \multicolumn{3}{c}{Accuracy} & \multicolumn{2}{c}{Attack robustness} \\
% \cmidrule(lr){1-2} \cmidrule(lr){3-5} \cmidrule(lr){6-7}
% \textbf{Trojan} & \multicolumn{1}{c}{\textbf{Train}} & ACC(\%)  & MS     & \multicolumn{1}{c}{ASR(\%)}  & BIR     & BRR  \\
% \midrule
% \multirow{1}{*}{BN}         & A-S    & 84.87	&0.57	&99.99	&1	&84 \\
% \multirow{1}{*}{BN}         & A-M    & 85.15	&0.86	&100	&34	&200+ \\
% \multirow{1}{*}{BN}         & A-BM   & 85.45	&0.95	&100	&54	&200+ \\
% \midrule
% \multirow{1}{*}{BL}         & A-S    & 84.97	&0.65	&100	&1	&57   \\
% \multirow{1}{*}{BL}         & A-M    & 84.54	&0.95	&100	&54	&200+ \\
% \multirow{1}{*}{BL}         & A-BM   & 84.44	&1.71	&100	&121	&200+ \\
% \midrule
% \multirow{1}{*}{DB}         & A-S    & 84.4	&0.16	&94.43	&5	&200+ \\
% \multirow{1}{*}{DB}         & A-M    & 85.34	&1.09	&98.4	&169	&\textbf{97} \\
% \bottomrule
% \end{tabular}
% \label{tab:fea_cla_t}
% \vspace{-4mm}
% \end{table}


  
% Note that, the comprehensive evaluation for defenses against untargeted attacks is in Sec.~\ref{subsec:un_attack_detection}.
% \begin{table*}[htbp]
% \centering
%   \footnotesize
%   \caption{Effectiveness of existing detection methods on CIFAR10 (ResNet18) in non-IID settings}
%   \vspace{-2mm}
% %   \resizebox{\linewidth}{!}{
% \begin{tabular}{@{}c|ccc||cccccccc@{}}
% \toprule
%  &
%   \multicolumn{3}{c||}{Untargeted Classical Attacks} &
%   \multicolumn{8}{c}{Untargeted Evasion Attacks} \\ \cmidrule(l){2-12} 
% Defense &
%   \multicolumn{1}{c|}{Add Noise} &
%   \multicolumn{1}{c|}{Sign-flipping} &
%   Dirty Label &
%   \begin{tabular}[c]{@{}c@{}}MTB\\ Mkrum\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}MTB\\ Bulyan\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}MTB\\ Median\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}MTB\\ Trmean\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}MTB\\ Min-Max\end{tabular} &
%   \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}MTB\\ Min-Sum\end{tabular}} &
%   \begin{tabular}[c]{@{}c@{}}Fang\\ Mkrum\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}Fang\\ Trmean\end{tabular} \\ \midrule
% \begin{tabular}[c]{@{}c@{}}Median \end{tabular} &
%   \multicolumn{1}{c|}{High} &  \multicolumn{1}{c|}{High} &  High &  High &  High &  High &  High &  High &  \multicolumn{1}{c|}{High} &  High &  High \\
% DnC &
%   \multicolumn{1}{c|}{Low} &  \multicolumn{1}{c|}{High} &  High &  High &  High &  Low &  Low &  High &  \multicolumn{1}{c|}{High} &  High &  High \\ \bottomrule
% \end{tabular}
% % }
% \label{tab:resist_un}
% \vspace{-3mm}
% \end{table*}

% \begin{table*}[htbp]
%   \centering
%   \footnotesize
%   \caption{Effectiveness of existing detection methods against targeted attacks}
%   \vspace{-2mm}
%   \resizebox{\linewidth}{!}{
%     \begin{tabular}{c|ccc|ccc|cc||ccc|ccc|cc}
%     \toprule
%           & \multicolumn{8}{c||}{Targeted Classical Attacks}                                & \multicolumn{8}{c}{Targeted Evasion Attacks} \\ %\cmidrule(lr){2-9} \cmidrule(lr){10-17}
% \cmidrule{2-17}   & BN    & BN    & BN    & BL    & BL    & BL    & DB    & DB    & BN    & BN    & BN    & BL    & BL    & BL    & DB    & DB \\
%     Defense & A-S   & A-M   & A-BM  & A-S   & A-M   & A-BM  & A-S   & A-M   & A-S   & A-M   & A-BM  & A-S   & A-M   & A-BM  & A-S   & A-M \\
%     \midrule
%     DnC   &  Low&Low&High&Low&Low&High&Low&Low&Low&High&High&Low&High&High&Low&Median  \\
%     Fine-purning & High&High&High&Median&Median&Median&High&Median&High&High&High&High&High&High&High&High  \\
%     \bottomrule
%     \end{tabular}%
% }
%   \label{tab:resist_tar}%
%   \vspace{-3mm}
% \end{table*}%



% \subsection{Analysis and Takeaways}\label{sec:takeaway}
% Here, we summarize some knowledge revealed by our experimental studies, including limitations of existing detection methods for poisoning attacks and 
% % , the reason why CRBA attack is effective, and limitations of random noise trigger (BL).

% \textbf{Existing defense schemes have high false positives, which leads to a lack of unique data for training.}
% Gradient anomaly defense algorithms misclassify benign updates as malicious in non-IID settings. This is because the feature distribution and label distribution of non-IID clients are skewed and the clustering algorithm cannot distinguish non-IID data from malicious data. In addition, misclassified clients are misclassified almost every participation round, as shown in Table~\ref{tab:targeted_attack_detection_noniid}.\footnote{We have discussed with the authors~\cite{shejwalkar2021manipulating} to confirm the results.} This means that their unique data can never be involved in the training. This is a serious data deficit for FL. 
% % (Since Byzantine-robust aggregation algorithms detect well on add noise attack, no further detection is required.)
% % Removing the noniid data at different stages of training has different effects on the main task. As shown in Fig.~\ref{fig:acc_t_cifar_backdoor}, we remove the most abnormal data with pca during normal training. Before 100 rounds, the accuracy is higher than that of using all updates. However, after 100 rounds, the main task requires more diverse data, so combining all updates is more accurate. 

% \textbf{Existing defense schemes against targeted attacks can be evaded by the replacement of weights of convolution layers.}
% 

% !!!!!!!!!!!!!!!!!!!!!!!
% \textbf{Random noise trigger (BL) is vulnerable on FL.} BL is added into input samples with certain transparency, where the level of attack effect increases with decreasing patterns transparency. There exist a trade-off between effect and transparency. However, for perturbation triggers with low transparency, there is low resolution for the clean input sample and high perceptibility of the trigger to human beings, which contravene the stealthy objective of backdoor attacks. Therefore, BL with high transparency leads to the attenuation of the attack effect, slowing down the implantation process and weakening the stability of the backdoor. Although trigger size has a positive effect on the attack effect, BL of the full image has a lower backdoor implantation speed compared to an opaque patch trigger (BN) due to high transparency. The results of backdoor injection with BL and BN are shown in the Appendix~\ref{fig:acc_backdoor_cifar}.


% \textbf{Single-shot attack of distributed pattern is more robust than multi-shot attack. While in other types of patterns, multi-shot attack is more robust than single-shot attack.} 
% As shown in 

% \begin{figure}[h]
%   \centering
%       \includegraphics[width=0.8\linewidth]{./figures/acc_backdoor_cifar_DBA}
%   \caption{DBA Training in ResNet18 with Different Strategies.}
%   \label{fig:acc_backdoor_cifar_DBA}
% \end{figure}

% \begin{table}[]
% \caption{Main Task and Backdoor Task Accuracy in Different Backdoor Attacks}
% \begin{tabular}{ccc}
% \toprule
%  & Main Task & Backdoor Task \\ \midrule
% $\{w_r^*, b_r^*, w_c^*, b_c^*\}$  & 67\%   & 100\%   \\
% $\{w_r^*, b_r, w_c, b_c\}$ & 68\%  & 99\%  \\
% $\{w_r, b_r^*, w_c^*, b_c^*\}$ & 68\%  & 10\% \\ \bottomrule
% \end{tabular}
% \end{table}




% Accuracy (\textit{ACC}) and Attack Success Rate (\textit{ASR}) are two macro-level metrics for the evaluation of poisoning attacks. Then we introduce four new metrics to describe untargeted attack performance in detail: Model Stability (\textit{MS}), Worst/Best Category Accuracy (\textit{WCA/BCA}) and Category\ Accuracy\ Stability (\textit{CAS}). We introduce two new metrics to describe targeted attack performance in detail: Backdoor Injection Rounds (\textit{BIR}) and Backdoor Duration Rounds (\textit{BRR}).

% \uline{Accuracy} (\textit{ACC}) - which is the classification accuracy of the global model. For untargeted attacks, a lower \textit{ACC} indicates an effective attack. For targeted attacks, a higher \textit{ACC} indicates that backdoor injection has less impact on the classification accuracy of the global model.

% \uline{Attack Success Rate} (\textit{ASR}) - which is the attack success rate of the targeted poisoning attack. It measures the likelihood of the trigger input being classified as a target category. An attack with a higher \textit{ASR} is more effective. 

% \uline{Model Stability} (\textit{MS}) - which measures the stability of the model on the classification task. It is the standard deviation of the model accuracy in the last ten rounds: 
% $$MS=\sqrt{\frac{1}{10}\sum_{r\in[\rho]}(ACC^r-\overline{ACC})^2}$$ %\mathrm{Model\ Stability}
% where $[\rho]$ is the last ten rounds and $\overline{ACC}$ is the average of \textit{ACC} in the last ten rounds. A higher \textit{MS} indicates more effective untargetd attacks. 

% \uline{Worst/Best Category Accuracy} (\textit{WCA/BCA}) - which are the highest and lowest values of the category accuracy:  
% \begin{equation}
% \begin{aligned}
% CA_c=\frac{\mathrm{\#\ Correct\ predictions\ of\ category}\ c}{\mathrm{\#\ Total\ predictions\ of\ category}\ c} \\ %\mathrm{Category\ Accuracy}
% WCA=\min\limits_{c\in[m]} CA_c \qquad BCA=\max\limits_{c\in[m]} CA_c %\mathrm{Worst\ CA}, \mathrm{Best\ CA}
% \nonumber
% \end{aligned}
% \end{equation} 
% %
% where $m$ is the number of categories. Due to the imbalance of various types of data on FL, it is necessary to maintain the accuracy of all categories. 

% \uline{Category\ Accuracy\ Stability} (\textit{CAS}) - which measures the stability of category accuracy. It is the standard deviation of all category accuracies in the last te rounds:
% $$CAS=\sqrt{\frac{1}{10}\sum_{r\in[\rho],c\in[m]}(CA_c^r-\overline{CA})^2}$$
% A higer $CAS$ indicates a more effective untargeted attack.

% \uline{Backdoor Injection Rounds} (\textit{BIR}) - is the number of rounds from the start of the attack to the \textit{ASR} of 99\%. A smaller \textit{BIR} indicates an effective backdoor attack.

% \uline{Backdoor Duration Rounds} (\textit{BRR}) - which measures the stability of the trojan model. We first test a model with trigger inputs and obtain the \textit{ASR} as a benchmark for this backdoor attack. We then train a trojan model with benign clients as if it were trained normally without an adversary. The number of rounds required to reduce a high \textit{ASR} to the benchmark is \textit{BRR}. Normally the benchmark is 10\%, while for BL Trigger, benchmark is 23.9\%. This is because the additive random noise in BL modifies the clean images significantly, which makes the benign model misclassified.



==> bio.tex <==
\newpage

\section*{Biography Section}
If you have an EPS/PDF photo (graphicx package needed), extra braces are
 needed around the contents of the optional argument to biography to prevent
 the LaTeX parser from getting confused when it sees the complicated
 $\backslash${\tt{includegraphics}} command within an optional argument. (You can create
 your own custom macro containing the $\backslash${\tt{includegraphics}} command to make things
 simpler here.)
 
\vspace{11pt}

\bf{If you include a photo:}\vspace{-33pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig1}}]{Michael Shell}
Use $\backslash${\tt{begin\{IEEEbiography\}}} and then for the 1st argument use $\backslash${\tt{includegraphics}} to declare and link the author photo.
Use the author name as the 3rd argument followed by the biography text.
\end{IEEEbiography}

\vspace{11pt}

\bf{If you will not include a photo:}\vspace{-33pt}
\begin{IEEEbiographynophoto}{John Doe}
Use $\backslash${\tt{begin\{IEEEbiographynophoto\}}} and the author name as the argument followed by the biography text.
\end{IEEEbiographynophoto}




\vfill
